A Comparison of the Embedding Method to Multi-Parametric Programming, Mixed-Integer Programming, Gradient-Descent, and Hybrid Minimum Principle Based Methods

In recent years, the embedding approach for solving switched optimal control problems has been developed in a series of papers. However, the embedding approach, which advantageously converts the hybrid optimal control problem to a classical nonlinear optimization, has not been extensively compared to alternative solution approaches. The goal of this paper is thus to compare the embedding approach to multi-parametric programming, mixed-integer programming (e.g., CPLEX), and gradient-descent based methods in the context of five recently published examples: a spring-mass system, moving-target tracking for a mobile robot, two-tank filling, DC-DC boost converter, and skid-steered vehicle. A sixth example, an autonomous switched 11-region linear system, is used to compare a hybrid minimum principle method and traditional numerical programming. For a given performance index for each case, cost and solution times are presented. It is shown that there are numerical advantages of the embedding approach: lower performance index cost (except in some instances when autonomous switches are present), generally faster solution time, and convergence to a solution when other methods may fail. In addition, the embedding method requires no ad hoc assumptions (e.g., predetermined mode sequences) or specialized control models. Theoretical advantages of the embedding approach over the other methods are also described: guaranteed existence of a solution under mild conditions, convexity of the embedded hybrid optimization problem (under the customary conditions on the performance index), solvability with traditional techniques (e.g., sequential quadratic programming) avoiding the combinatorial complexity in the number of modes/discrete variables of mixed-integer programming, applicability to affine nonlinear systems, and no need to explicitly assign discrete/mode variables to autonomous switches.

==> f-boostconverter-eoc-cplex-states-dc.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{f-boostconverter-eoc-cplex-states-dc}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           11-Apr-2012 09:51:06
% eps bounding box:     10 cm x 7.5 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s09}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_o(t)$\end{tabular}}%
\psfrag{s10}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$i_L(t)$\end{tabular}}%
\psfrag{s11}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Duty Cycle\end{tabular}}%
\psfrag{s12}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time (ms)\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{5}%
\psfrag{x03}[t][t]{10}%
\psfrag{x04}[t][t]{15}%
\psfrag{x05}[t][t]{20}%
\psfrag{x06}[t][t]{25}%
\psfrag{x07}[t][t]{30}%
\psfrag{x08}[t][t]{35}%
\psfrag{x09}[t][t]{40}%
\psfrag{x10}[t][t]{45}%
\psfrag{x11}[t][t]{50}%
\psfrag{x12}[t][t]{0}%
\psfrag{x13}[t][t]{5}%
\psfrag{x14}[t][t]{10}%
\psfrag{x15}[t][t]{15}%
\psfrag{x16}[t][t]{20}%
\psfrag{x17}[t][t]{25}%
\psfrag{x18}[t][t]{30}%
\psfrag{x19}[t][t]{35}%
\psfrag{x20}[t][t]{40}%
\psfrag{x21}[t][t]{45}%
\psfrag{x22}[t][t]{50}%
\psfrag{x23}[t][t]{0}%
\psfrag{x24}[t][t]{5}%
\psfrag{x25}[t][t]{10}%
\psfrag{x26}[t][t]{15}%
\psfrag{x27}[t][t]{20}%
\psfrag{x28}[t][t]{25}%
\psfrag{x29}[t][t]{30}%
\psfrag{x30}[t][t]{35}%
\psfrag{x31}[t][t]{40}%
\psfrag{x32}[t][t]{45}%
\psfrag{x33}[t][t]{50}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.5}%
\psfrag{v03}[r][r]{1}%
\psfrag{v04}[r][r]{-5}%
\psfrag{v05}[r][r]{0}%
\psfrag{v06}[r][r]{5}%
\psfrag{v07}[r][r]{20}%
\psfrag{v08}[r][r]{40}%
\psfrag{v09}[r][r]{60}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{f-boostconverter-eoc-cplex-states-dc.eps}}%
\end{psfrags}%
%
% End f-boostconverter-eoc-cplex-states-dc.tex


==> f-boostconverter-states-dc.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{f-boostconverter-states-dc}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           03-Mar-2012 15:28:55
% eps bounding box:     10 cm x 7.5 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s09}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$v_o(t)$\end{tabular}}%
\psfrag{s10}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$i_L(t)$\end{tabular}}%
\psfrag{s11}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Duty Cycle\end{tabular}}%
\psfrag{s12}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time (ms)\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{5}%
\psfrag{x03}[t][t]{10}%
\psfrag{x04}[t][t]{15}%
\psfrag{x05}[t][t]{20}%
\psfrag{x06}[t][t]{25}%
\psfrag{x07}[t][t]{30}%
\psfrag{x08}[t][t]{35}%
\psfrag{x09}[t][t]{40}%
\psfrag{x10}[t][t]{45}%
\psfrag{x11}[t][t]{50}%
\psfrag{x12}[t][t]{0}%
\psfrag{x13}[t][t]{5}%
\psfrag{x14}[t][t]{10}%
\psfrag{x15}[t][t]{15}%
\psfrag{x16}[t][t]{20}%
\psfrag{x17}[t][t]{25}%
\psfrag{x18}[t][t]{30}%
\psfrag{x19}[t][t]{35}%
\psfrag{x20}[t][t]{40}%
\psfrag{x21}[t][t]{45}%
\psfrag{x22}[t][t]{50}%
\psfrag{x23}[t][t]{0}%
\psfrag{x24}[t][t]{5}%
\psfrag{x25}[t][t]{10}%
\psfrag{x26}[t][t]{15}%
\psfrag{x27}[t][t]{20}%
\psfrag{x28}[t][t]{25}%
\psfrag{x29}[t][t]{30}%
\psfrag{x30}[t][t]{35}%
\psfrag{x31}[t][t]{40}%
\psfrag{x32}[t][t]{45}%
\psfrag{x33}[t][t]{50}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{0.5}%
\psfrag{v03}[r][r]{1}%
\psfrag{v04}[r][r]{-2}%
\psfrag{v05}[r][r]{0}%
\psfrag{v06}[r][r]{2}%
\psfrag{v07}[r][r]{20}%
\psfrag{v08}[r][r]{40}%
\psfrag{v09}[r][r]{60}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{f-boostconverter-states-dc.eps}}%
\end{psfrags}%
%
% End f-boostconverter-states-dc.tex


==> f-eoc-11mode-states-automode-Hp=80-cont.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{f-eoc-11mode-states-automode}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           30-Mar-2012 10:11:26
% eps bounding box:     10 cm x 7.5 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s09}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$x_1(t)$\end{tabular}}%
\psfrag{s10}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$x_2(t)$\end{tabular}}%
\psfrag{s11}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}q(t)\end{tabular}}%
\psfrag{s12}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}Time (s)\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{0}%
\psfrag{x02}[t][t]{0.2}%
\psfrag{x03}[t][t]{0.4}%
\psfrag{x04}[t][t]{0.6}%
\psfrag{x05}[t][t]{0.8}%
\psfrag{x06}[t][t]{1}%
\psfrag{x07}[t][t]{1.2}%
\psfrag{x08}[t][t]{1.4}%
\psfrag{x09}[t][t]{1.6}%
\psfrag{x10}[t][t]{1.8}%
\psfrag{x11}[t][t]{2}%
\psfrag{x12}[t][t]{0}%
\psfrag{x13}[t][t]{0.2}%
\psfrag{x14}[t][t]{0.4}%
\psfrag{x15}[t][t]{0.6}%
\psfrag{x16}[t][t]{0.8}%
\psfrag{x17}[t][t]{1}%
\psfrag{x18}[t][t]{1.2}%
\psfrag{x19}[t][t]{1.4}%
\psfrag{x20}[t][t]{1.6}%
\psfrag{x21}[t][t]{1.8}%
\psfrag{x22}[t][t]{2}%
\psfrag{x23}[t][t]{0}%
\psfrag{x24}[t][t]{0.2}%
\psfrag{x25}[t][t]{0.4}%
\psfrag{x26}[t][t]{0.6}%
\psfrag{x27}[t][t]{0.8}%
\psfrag{x28}[t][t]{1}%
\psfrag{x29}[t][t]{1.2}%
\psfrag{x30}[t][t]{1.4}%
\psfrag{x31}[t][t]{1.6}%
\psfrag{x32}[t][t]{1.8}%
\psfrag{x33}[t][t]{2}%
%
% yticklabels:
\psfrag{v01}[r][r]{0}%
\psfrag{v02}[r][r]{5}%
\psfrag{v03}[r][r]{10}%
\psfrag{v04}[r][r]{-10}%
\psfrag{v05}[r][r]{-5}%
\psfrag{v06}[r][r]{0}%
\psfrag{v07}[r][r]{5}%
\psfrag{v08}[r][r]{-10}%
\psfrag{v09}[r][r]{-5}%
\psfrag{v10}[r][r]{0}%
\psfrag{v11}[r][r]{5}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{f-eoc-11mode-states-automode.eps}}%
\end{psfrags}%
%
% End f-eoc-11mode-states-automode.tex


==> f-eoc-11mode-statespace-Hp=80-cont.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{f-eoc-11mode-statespace}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           30-Mar-2012 10:10:49
% eps bounding box:     10 cm x 7.5 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s03}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}1\end{tabular}}%
\psfrag{s04}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}2\end{tabular}}%
\psfrag{s05}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}3\end{tabular}}%
\psfrag{s06}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}4\end{tabular}}%
\psfrag{s07}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}5\end{tabular}}%
\psfrag{s08}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}6\end{tabular}}%
\psfrag{s09}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}7\end{tabular}}%
\psfrag{s10}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}8\end{tabular}}%
\psfrag{s11}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}9\end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}10\end{tabular}}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}11\end{tabular}}%
\psfrag{s14}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$x_2(t)$\end{tabular}}%
\psfrag{s15}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$x_1(t)$\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-10}%
\psfrag{x02}[t][t]{-5}%
\psfrag{x03}[t][t]{0}%
\psfrag{x04}[t][t]{5}%
%
% yticklabels:
\psfrag{v01}[r][r]{-8}%
\psfrag{v02}[r][r]{-6}%
\psfrag{v03}[r][r]{-4}%
\psfrag{v04}[r][r]{-2}%
\psfrag{v05}[r][r]{0}%
\psfrag{v06}[r][r]{2}%
\psfrag{v07}[r][r]{4}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{f-eoc-11mode-statespace.eps}}%
\end{psfrags}%
%
% End f-eoc-11mode-statespace.tex


==> f-eoc-11mode-statespace-Hp=80-initguess.tex <==
% This file is generated by the MATLAB m-file laprint.m. It can be included
% into LaTeX documents using the packages graphicx, color and psfrag.
% It is accompanied by a postscript file. A sample LaTeX file is:
%    \documentclass{article}\usepackage{graphicx,color,psfrag}
%    \begin{document}\input{f-eoc-11mode-statespace-Hp=80-initguess}\end{document}
% See http://www.mathworks.de/matlabcentral/fileexchange/loadFile.do?objectId=4638
% for recent versions of laprint.m.
%
% created by:           LaPrint version 3.16 (13.9.2004)
% created on:           08-May-2012 09:47:10
% eps bounding box:     10 cm x 7.5 cm
% comment:              
%
\begin{psfrags}%
\psfragscanon%
%
% text strings:
\psfrag{s03}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}1\end{tabular}}%
\psfrag{s04}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}2\end{tabular}}%
\psfrag{s05}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}3\end{tabular}}%
\psfrag{s06}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}4\end{tabular}}%
\psfrag{s07}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}5\end{tabular}}%
\psfrag{s08}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}6\end{tabular}}%
\psfrag{s09}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}7\end{tabular}}%
\psfrag{s10}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}8\end{tabular}}%
\psfrag{s11}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}9\end{tabular}}%
\psfrag{s12}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}10\end{tabular}}%
\psfrag{s13}[l][l]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{l}11\end{tabular}}%
\psfrag{s14}[b][b]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$x_2(t)$\end{tabular}}%
\psfrag{s15}[t][t]{\color[rgb]{0,0,0}\setlength{\tabcolsep}{0pt}\begin{tabular}{c}$x_1(t)$\end{tabular}}%
%
% xticklabels:
\psfrag{x01}[t][t]{-10}%
\psfrag{x02}[t][t]{-5}%
\psfrag{x03}[t][t]{0}%
\psfrag{x04}[t][t]{5}%
%
% yticklabels:
\psfrag{v01}[r][r]{-8}%
\psfrag{v02}[r][r]{-6}%
\psfrag{v03}[r][r]{-4}%
\psfrag{v04}[r][r]{-2}%
\psfrag{v05}[r][r]{0}%
\psfrag{v06}[r][r]{2}%
\psfrag{v07}[r][r]{4}%
%
% Figure:
\resizebox{8cm}{!}{\includegraphics{f-eoc-11mode-statespace-Hp=80-initguess.eps}}%
\end{psfrags}%
%
% End f-eoc-11mode-statespace-Hp=80-initguess.tex

